Measuring GPU Memory Traffic on the NVIDIA GB10 Without C2C Telemetry

The NVIDIA GB10, used in the DGX Spark and in desktop AI systems from several vendors, joins an Arm CPU die and a Blackwell GPU die with NVLink C2C. The GPU has no local memory, so every GPU access that misses in its L2 cache crosses C2C to the LPDDR5X attached to the CPU die. Yet the software on the systems we tested exposes no counter for this traffic. We show that five L2 sector counters of the GPU, sampled every 10 ms through NVIDIA's CUPTI sampling interface by a process that does not attach to the workload, measure GPU memory traffic live and separate copy engine traffic from the read misses and writes of GPU kernels. For large streaming transfers of known size, the counters agree within 0.28% on an Acer GN100 and within 0.005% on a DGX Spark, track the volume moved regardless of how it is split into copies, and exclude data reused in L2. The GPU's SMMU counter, a natural alternative, counts address translations rather than bytes. Applied to an unmodified server, the method shows Mistral 7B decode reading 13.47 GiB per token, the weights it uses plus its key value (KV) cache, at 83% of the memory bandwidth NVIDIA specifies. We release the method as an open source tool.

==> values.tex <==
% AUTO-GENERATED by scripts/make_values.py from data/*.csv. Do not edit.
\makeatletter
\newcommand{\val}[1]{\@ifundefined{val@#1}{\textbf{??\detokenize{#1}??}}{\csname val@#1\endcsname}}
\expandafter\def\csname val@buf.l2_ratio\endcsname{11}
\expandafter\def\csname val@cal.bytes_per_txn\endcsname{2,098}
\expandafter\def\csname val@cal.cv_max\endcsname{2.7}
\expandafter\def\csname val@cal.d2h.bytes_hi\endcsname{2,116}
\expandafter\def\csname val@cal.d2h.bytes_lo\endcsname{2,083}
\expandafter\def\csname val@cal.d2h.bytes_per_txn\endcsname{2,099}
\expandafter\def\csname val@cal.d2h.cv_max\endcsname{2.7}
\expandafter\def\csname val@cal.d2h.intercept\endcsname{187,494}
\expandafter\def\csname val@cal.d2h.per_round\endcsname{127,857}
\expandafter\def\csname val@cal.d2h.per_round_ci\endcsname{993}
\expandafter\def\csname val@cal.d2h.r2\endcsname{0.9998}
\expandafter\def\csname val@cal.dir_diff\endcsname{0.1}
\expandafter\def\csname val@cal.h2d.bytes_hi\endcsname{2,112}
\expandafter\def\csname val@cal.h2d.bytes_lo\endcsname{2,081}
\expandafter\def\csname val@cal.h2d.bytes_per_txn\endcsname{2,097}
\expandafter\def\csname val@cal.h2d.cv_max\endcsname{2.0}
\expandafter\def\csname val@cal.h2d.intercept\endcsname{169,600}
\expandafter\def\csname val@cal.h2d.per_round\endcsname{128,027}
\expandafter\def\csname val@cal.h2d.per_round_ci\endcsname{936}
\expandafter\def\csname val@cal.h2d.r2\endcsname{0.9998}
\expandafter\def\csname val@cal.intercept_k\endcsname{179}
\expandafter\def\csname val@cal.intercept_raw_k\endcsname{200}
\expandafter\def\csname val@cal.max_gib\endcsname{8}
\expandafter\def\csname val@cal.r2_min\endcsname{0.9998}
\expandafter\def\csname val@cal.repeats\endcsname{5}
\expandafter\def\csname val@checks.all\endcsname{pass}
\expandafter\def\csname val@gemm.inputs_mib\endcsname{64}
\expandafter\def\csname val@gemm.mb\endcsname{211}
\expandafter\def\csname val@gemm.n\endcsname{4096}
\expandafter\def\csname val@gemm.reuse\endcsname{3.1}
\expandafter\def\csname val@gemm.sectors\endcsname{6,598,719}
\expandafter\def\csname val@idle.rate\endcsname{36,329}
\expandafter\def\csname val@idle.rate_sd\endcsname{24,763}
\expandafter\def\csname val@idle.source\endcsname{measured}
\expandafter\def\csname val@ip.copied_mib\endcsname{2,048}
\expandafter\def\csname val@ip.id\endcsname{pravaha-calibrate\_2026-11-05T04:51}
\expandafter\def\csname val@ip.idle.rate\endcsname{3,625}
\expandafter\def\csname val@ip.idle.rate_sd\endcsname{1,768}
\expandafter\def\csname val@ip.level_spread_max\endcsname{2.8}
\expandafter\def\csname val@ip.max\endcsname{3,842}
\expandafter\def\csname val@ip.min\endcsname{2,089}
\expandafter\def\csname val@ip.n_unstable\endcsname{1}
\expandafter\def\csname val@ip.pageable.max_mib\endcsname{256}
\expandafter\def\csname val@ip.pageable.min_mib\endcsname{4}
\expandafter\def\csname val@ip.pageable_256.bpt\endcsname{3,769}
\expandafter\def\csname val@ip.pageable_256.hi\endcsname{3,796}
\expandafter\def\csname val@ip.pageable_256.lo\endcsname{3,769}
\expandafter\def\csname val@ip.pageable_256.spread\endcsname{0.7}
\expandafter\def\csname val@ip.pageable_4.bpt\endcsname{3,693}
\expandafter\def\csname val@ip.pageable_4.hi\endcsname{3,693}
\expandafter\def\csname val@ip.pageable_4.lo\endcsname{3,685}
\expandafter\def\csname val@ip.pageable_4.spread\endcsname{0.2}
\expandafter\def\csname val@ip.pageable_64.bpt\endcsname{3,842}
\expandafter\def\csname val@ip.pageable_64.hi\endcsname{3,842}
\expandafter\def\csname val@ip.pageable_64.lo\endcsname{3,842}
\expandafter\def\csname val@ip.pageable_64.spread\endcsname{0.0}
\expandafter\def\csname val@ip.pinned.max_mib\endcsname{256}
\expandafter\def\csname val@ip.pinned.min_mib\endcsname{1}
\expandafter\def\csname val@ip.pinned_1.bpt\endcsname{3,450}
\expandafter\def\csname val@ip.pinned_1.hi\endcsname{3,461}
\expandafter\def\csname val@ip.pinned_1.lo\endcsname{3,375}
\expandafter\def\csname val@ip.pinned_1.spread\endcsname{2.5}
\expandafter\def\csname val@ip.pinned_128.bpt\endcsname{3,121}
\expandafter\def\csname val@ip.pinned_128.hi\endcsname{3,121}
\expandafter\def\csname val@ip.pinned_128.level_hi\endcsname{3,121}
\expandafter\def\csname val@ip.pinned_128.level_lo\endcsname{2,261}
\expandafter\def\csname val@ip.pinned_128.lo\endcsname{2,261}
\expandafter\def\csname val@ip.pinned_128.n_between\endcsname{1}
\expandafter\def\csname val@ip.pinned_128.n_hi\endcsname{6}
\expandafter\def\csname val@ip.pinned_128.n_lo\endcsname{3}
\expandafter\def\csname val@ip.pinned_128.spread\endcsname{27.6}
\expandafter\def\csname val@ip.pinned_16.bpt\endcsname{3,842}
\expandafter\def\csname val@ip.pinned_16.hi\endcsname{3,845}
\expandafter\def\csname val@ip.pinned_16.lo\endcsname{3,833}
\expandafter\def\csname val@ip.pinned_16.spread\endcsname{0.3}
\expandafter\def\csname val@ip.pinned_2.bpt\endcsname{3,747}
\expandafter\def\csname val@ip.pinned_2.hi\endcsname{3,831}
\expandafter\def\csname val@ip.pinned_2.lo\endcsname{3,738}
\expandafter\def\csname val@ip.pinned_2.spread\endcsname{2.5}
\expandafter\def\csname val@ip.pinned_256.bpt\endcsname{2,089}
\expandafter\def\csname val@ip.pinned_256.hi\endcsname{2,089}
\expandafter\def\csname val@ip.pinned_256.lo\endcsname{2,087}
\expandafter\def\csname val@ip.pinned_256.spread\endcsname{0.1}
\expandafter\def\csname val@ip.pinned_32.bpt\endcsname{3,803}
\expandafter\def\csname val@ip.pinned_32.hi\endcsname{3,806}
\expandafter\def\csname val@ip.pinned_32.lo\endcsname{3,795}
\expandafter\def\csname val@ip.pinned_32.spread\endcsname{0.3}
\expandafter\def\csname val@ip.pinned_4.bpt\endcsname{3,800}
\expandafter\def\csname val@ip.pinned_4.hi\endcsname{3,824}
\expandafter\def\csname val@ip.pinned_4.lo\endcsname{3,717}
\expandafter\def\csname val@ip.pinned_4.spread\endcsname{2.8}
\expandafter\def\csname val@ip.pinned_64.bpt\endcsname{2,558}
\expandafter\def\csname val@ip.pinned_64.hi\endcsname{2,620}
\expandafter\def\csname val@ip.pinned_64.lo\endcsname{2,557}
\expandafter\def\csname val@ip.pinned_64.spread\endcsname{2.5}
\expandafter\def\csname val@ip.pinned_8.bpt\endcsname{3,828}
\expandafter\def\csname val@ip.pinned_8.hi\endcsname{3,829}
\expandafter\def\csname val@ip.pinned_8.lo\endcsname{3,825}
\expandafter\def\csname val@ip.pinned_8.spread\endcsname{0.1}
\expandafter\def\csname val@ip.ratio\endcsname{1.8}
\expandafter\def\csname val@ip.repeats\endcsname{5}
\expandafter\def\csname val@ip.unstable\endcsname{128~MiB}
\expandafter\def\csname val@ip.unstable_pct\endcsname{5}
\expandafter\def\csname val@kern.device.delta8\endcsname{6,100}
\expandafter\def\csname val@kern.expected_per8\endcsname{1,023,539}
\expandafter\def\csname val@kern.malloc.delta8\endcsname{69,875}
\expandafter\def\csname val@kern.max_delta8\endcsname{69,875}
\expandafter\def\csname val@kern.max_delta8_pct\endcsname{7}
\expandafter\def\csname val@kern.pinned.delta8\endcsname{62,818}
\expandafter\def\csname val@plat.bios\endcsname{5.36\_0ACUM05}
\expandafter\def\csname val@plat.c2c_agg_gbps\endcsname{600}
\expandafter\def\csname val@plat.compute_capability\endcsname{12.1}
\expandafter\def\csname val@plat.concurrent_managed_access\endcsname{1}
\expandafter\def\csname val@plat.cuda_driver_api\endcsname{13.0}
\expandafter\def\csname val@plat.cuda_runtime\endcsname{13.0}
\expandafter\def\csname val@plat.date\endcsname{2026-11-04}
\expandafter\def\csname val@plat.dcgm\endcsname{}
\expandafter\def\csname val@plat.dcgm_tested\endcsname{3.3.9 and 4.7.1}
\expandafter\def\csname val@plat.driver\endcsname{580.159.03}
\expandafter\def\csname val@plat.gpu_name\endcsname{NVIDIA GB10}
\expandafter\def\csname val@plat.gpu_pci\endcsname{000f:01:00.0}
\expandafter\def\csname val@plat.gpu_pci_raw\endcsname{0000000F:01:00.0}
\expandafter\def\csname val@plat.integrated\endcsname{1}
\expandafter\def\csname val@plat.kernel\endcsname{6.17.0-1021-nvidia}
\expandafter\def\csname val@plat.l2_bytes\endcsname{25165824}
\expandafter\def\csname val@plat.l2_mib\endcsname{24}
\expandafter\def\csname val@plat.machine\endcsname{Acer GN100 (NVIDIA GB10)}
\expandafter\def\csname val@plat.memory_gb\endcsname{128}
\expandafter\def\csname val@plat.ncu\endcsname{2025.3.1.0}
\expandafter\def\csname val@plat.nvcc\endcsname{13.0}
\expandafter\def\csname val@plat.os\endcsname{Ubuntu 24.04.4 LTS}
\expandafter\def\csname val@plat.pageable_access\endcsname{1}
\expandafter\def\csname val@plat.perf\endcsname{6.17.13}
\expandafter\def\csname val@plat.repeats\endcsname{5}
\expandafter\def\csname val@plat.sampling_ms\endcsname{100}
\expandafter\def\csname val@plat.sm_count\endcsname{48}
\expandafter\def\csname val@plat.unit\endcsname{smmuv3\_pmcg\_13002}
\expandafter\def\csname val@plat.uses_host_page_tables\endcsname{1}
\expandafter\def\csname val@plat.vbios\endcsname{9A.0B.0F.00.1D}
\expandafter\def\csname val@rd.device.device\endcsname{0}
\expandafter\def\csname val@rd.device.err\endcsname{0.09}
\expandafter\def\csname val@rd.device.sectors\endcsname{8,395,898}
\expandafter\def\csname val@rd.err_max\endcsname{0.33}
\expandafter\def\csname val@rd.malloc.device\endcsname{0}
\expandafter\def\csname val@rd.malloc.err\endcsname{0.33}
\expandafter\def\csname val@rd.malloc.sectors\endcsname{8,416,100}
\expandafter\def\csname val@rd.mode_spread\endcsname{0.24}
\expandafter\def\csname val@rd.pinned.device\endcsname{0}
\expandafter\def\csname val@rd.pinned.err\endcsname{0.22}
\expandafter\def\csname val@rd.pinned.sectors\endcsname{8,407,084}
\expandafter\def\csname val@round.mib\endcsname{256}
\expandafter\def\csname val@scan.gpu.copy\endcsname{118,688,863}
\expandafter\def\csname val@scan.gpu.idle\endcsname{205,188}
\expandafter\def\csname val@scan.gpu.ratio\endcsname{578}
\expandafter\def\csname val@scan.n_units\endcsname{17}
\expandafter\def\csname val@sect.bytes\endcsname{32}
\expandafter\def\csname val@sect.expected\endcsname{8,388,608}
\expandafter\def\csname val@sz.max\endcsname{3,920}
\expandafter\def\csname val@sz.max_kib\endcsname{3.8}
\expandafter\def\csname val@sz.min\endcsname{2,158}
\expandafter\def\csname val@sz.min_kib\endcsname{2.1}
\expandafter\def\csname val@sz.pageable.max_mib\endcsname{256}
\expandafter\def\csname val@sz.pageable.min_mib\endcsname{4}
\expandafter\def\csname val@sz.pageable_256.bpt\endcsname{3,873}
\expandafter\def\csname val@sz.pageable_256.dev\endcsname{84.6}
\expandafter\def\csname val@sz.pageable_256.sd\endcsname{199}
\expandafter\def\csname val@sz.pageable_4.bpt\endcsname{3,663}
\expandafter\def\csname val@sz.pageable_4.dev\endcsname{74.6}
\expandafter\def\csname val@sz.pageable_4.sd\endcsname{53}
\expandafter\def\csname val@sz.pageable_64.bpt\endcsname{3,920}
\expandafter\def\csname val@sz.pageable_64.dev\endcsname{86.8}
\expandafter\def\csname val@sz.pageable_64.sd\endcsname{155}
\expandafter\def\csname val@sz.pinned.max_mib\endcsname{256}
\expandafter\def\csname val@sz.pinned.min_mib\endcsname{1}
\expandafter\def\csname val@sz.pinned_1.bpt\endcsname{3,468}
\expandafter\def\csname val@sz.pinned_1.dev\endcsname{65.3}
\expandafter\def\csname val@sz.pinned_1.sd\endcsname{235}
\expandafter\def\csname val@sz.pinned_128.bpt\endcsname{2,370}
\expandafter\def\csname val@sz.pinned_128.dev\endcsname{13.0}
\expandafter\def\csname val@sz.pinned_128.sd\endcsname{201}
\expandafter\def\csname val@sz.pinned_16.bpt\endcsname{3,891}
\expandafter\def\csname val@sz.pinned_16.dev\endcsname{85.5}
\expandafter\def\csname val@sz.pinned_16.sd\endcsname{65}
\expandafter\def\csname val@sz.pinned_2.bpt\endcsname{3,753}
\expandafter\def\csname val@sz.pinned_2.dev\endcsname{78.9}
\expandafter\def\csname val@sz.pinned_2.sd\endcsname{90}
\expandafter\def\csname val@sz.pinned_256.bpt\endcsname{2,158}
\expandafter\def\csname val@sz.pinned_256.dev\endcsname{2.9}
\expandafter\def\csname val@sz.pinned_256.sd\endcsname{56}
\expandafter\def\csname val@sz.pinned_32.bpt\endcsname{3,850}
\expandafter\def\csname val@sz.pinned_32.dev\endcsname{83.5}
\expandafter\def\csname val@sz.pinned_32.sd\endcsname{48}
\expandafter\def\csname val@sz.pinned_4.bpt\endcsname{3,802}
\expandafter\def\csname val@sz.pinned_4.dev\endcsname{81.2}
\expandafter\def\csname val@sz.pinned_4.sd\endcsname{34}
\expandafter\def\csname val@sz.pinned_64.bpt\endcsname{2,641}
\expandafter\def\csname val@sz.pinned_64.dev\endcsname{25.9}
\expandafter\def\csname val@sz.pinned_64.sd\endcsname{142}
\expandafter\def\csname val@sz.pinned_8.bpt\endcsname{3,846}
\expandafter\def\csname val@sz.pinned_8.dev\endcsname{83.3}
\expandafter\def\csname val@sz.pinned_8.sd\endcsname{86}
\expandafter\def\csname val@sz.ratio\endcsname{1.8}
\expandafter\def\csname val@trace.compute.start\endcsname{4.0}
\expandafter\def\csname val@trace.compute_mbps\endcsname{0}
\expandafter\def\csname val@trace.compute_w\endcsname{114.7}
\expandafter\def\csname val@trace.err\endcsname{26.5}
\expandafter\def\csname val@trace.idle.start\endcsname{10.0}
\expandafter\def\csname val@trace.idle_w\endcsname{14.0}
\expandafter\def\csname val@trace.known_gib\endcsname{4.00}
\expandafter\def\csname val@trace.load.start\endcsname{3.9}
\expandafter\def\csname val@trace.meas_gib\endcsname{5.06}
\expandafter\def\csname val@trace.offload.start\endcsname{10.0}
\expandafter\def\csname val@trace.other_gib\endcsname{0.36}
\expandafter\def\csname val@trace.peak_gbps\endcsname{22.4}
\expandafter\def\csname val@trace.phase_err\endcsname{4.5}
\expandafter\def\csname val@trace.phase_gib\endcsname{4.18}
\expandafter\def\csname val@trace.power_channel\endcsname{gpu}
\expandafter\def\csname val@trace.startup_gib\endcsname{0.52}
\expandafter\def\csname val@trace.tmax\endcsname{13}
\expandafter\def\csname val@wr.device.err\endcsname{0.05}
\expandafter\def\csname val@wr.device.fill\endcsname{3,565}
\expandafter\def\csname val@wr.device.fill_mb\endcsname{0}
\expandafter\def\csname val@wr.device.requests\endcsname{2,101,300}
\expandafter\def\csname val@wr.device.sectors\endcsname{8,392,778}
\expandafter\def\csname val@wr.err_max\endcsname{0.05}
\expandafter\def\csname val@wr.malloc.err\endcsname{15.25}
\expandafter\def\csname val@wr.malloc.fill\endcsname{3,383,439}
\expandafter\def\csname val@wr.malloc.fill_mb\endcsname{108}
\expandafter\def\csname val@wr.malloc.requests\endcsname{2,950,893}
\expandafter\def\csname val@wr.malloc.sectors\endcsname{9,667,528}
\expandafter\def\csname val@wr.pinned.err\endcsname{0.05}
\expandafter\def\csname val@wr.pinned.fill\endcsname{18,565}
\expandafter\def\csname val@wr.pinned.fill_mb\endcsname{1}
\expandafter\def\csname val@wr.pinned.requests\endcsname{2,101,127}
\expandafter\def\csname val@wr.pinned.sectors\endcsname{8,392,605}
\makeatother


==> values_v3.tex <==
% AUTO-GENERATED by scripts/make_values_v3.py from data/v3/. Do not edit.
\makeatletter
\providecommand{\val}[1]{\@ifundefined{val@#1}{\textbf{??\detokenize{#1}??}}{\csname val@#1\endcsname}}
\expandafter\def\csname val@all.l256.hi\endcsname{2,222}
\expandafter\def\csname val@all.l256.lo\endcsname{2,028}
\expandafter\def\csname val@all.l256.pct\endcsname{9.6}
\expandafter\def\csname val@all.n_campaigns\endcsname{4}
\expandafter\def\csname val@all.small.diff\endcsname{2.6}
\expandafter\def\csname val@gn.bg_rate\endcsname{3,388}
\expandafter\def\csname val@gn.bg_sd\endcsname{2,252}
\expandafter\def\csname val@gn.cal.big_hi\endcsname{2,620}
\expandafter\def\csname val@gn.cal.big_lo\endcsname{2,033}
\expandafter\def\csname val@gn.cal.method\endcsname{inprocess-2}
\expandafter\def\csname val@gn.cal.n_unstable\endcsname{3}
\expandafter\def\csname val@gn.cal.small_hi\endcsname{3,849}
\expandafter\def\csname val@gn.cal.small_lo\endcsname{3,642}
\expandafter\def\csname val@gn.cal_id\endcsname{pravaha-calibrate\_2026-11-08T03:42}
\expandafter\def\csname val@gn.cuda\endcsname{13.0}
\expandafter\def\csname val@gn.driver\endcsname{580.159.03}
\expandafter\def\csname val@gn.e4.bpt\endcsname{2,032}
\expandafter\def\csname val@gn.e4.dir_diff\endcsname{0.01}
\expandafter\def\csname val@gn.e4.r2\endcsname{0.9999}
\expandafter\def\csname val@gn.e6.device_pct\endcsname{0.6}
\expandafter\def\csname val@gn.e6.max_pct\endcsname{6.6}
\expandafter\def\csname val@gn.e7.malloc_extra_mb\endcsname{110}
\expandafter\def\csname val@gn.e7.malloc_w\endcsname{15.2}
\expandafter\def\csname val@gn.e7.read_max\endcsname{0.31}
\expandafter\def\csname val@gn.e7.write_max\endcsname{0.05}
\expandafter\def\csname val@gn.kernel\endcsname{6.17.0-1021-nvidia}
\expandafter\def\csname val@gn.n1.combined_err\endcsname{0.34}
\expandafter\def\csname val@gn.n1.copy_err\endcsname{0.59}
\expandafter\def\csname val@gn.n1.read_err\endcsname{0.14}
\expandafter\def\csname val@gn.n1.write_err\endcsname{0.08}
\expandafter\def\csname val@gn.n4.gb\endcsname{17.2}
\expandafter\def\csname val@gn.n4.max\endcsname{1,037}
\expandafter\def\csname val@gn.n4.min\endcsname{-4,249}
\expandafter\def\csname val@gn.n5.d2d\endcsname{-531}
\expandafter\def\csname val@gn.n5.d2h\endcsname{2,162}
\expandafter\def\csname val@gn.n5.h2d\endcsname{2,036}
\expandafter\def\csname val@gn.n6.bytes_per_txn\endcsname{2,029}
\expandafter\def\csname val@gn.n6.calibration\endcsname{2,057}
\expandafter\def\csname val@gn.n6.deviation_pct\endcsname{1.4}
\expandafter\def\csname val@gn.n6.run_spread_pct\endcsname{0.09}
\expandafter\def\csname val@gn.n6.status\endcsname{PASS}
\expandafter\def\csname val@gn.n6.tolerance_pct\endcsname{8.06}
\expandafter\def\csname val@gn.n7.max_pct\endcsname{0.17}
\expandafter\def\csname val@gn.n8.diff_pct\endcsname{0.01}
\expandafter\def\csname val@gn.n_boots\endcsname{2}
\expandafter\def\csname val@gn.n_campaigns\endcsname{3}
\expandafter\def\csname val@gn.n_candidates\endcsname{7}
\expandafter\def\csname val@gn.product\endcsname{Acer Veriton GN100}
\expandafter\def\csname val@gn.rerun.cpuonly\endcsname{yes}
\expandafter\def\csname val@gn.unit\endcsname{smmuv3\_pmcg\_13002}
\expandafter\def\csname val@live.err_max\endcsname{1.0}
\expandafter\def\csname val@live.gn.err_max\endcsname{1.01}
\expandafter\def\csname val@live.interval_us\endcsname{45}
\expandafter\def\csname val@live.run_spread_max\endcsname{6.1}
\expandafter\def\csname val@live.runs\endcsname{20}
\expandafter\def\csname val@live.sp.err_max\endcsname{0.19}
\expandafter\def\csname val@live.time_diff_max\endcsname{3.6}
\expandafter\def\csname val@sp.bg_rate\endcsname{2,792}
\expandafter\def\csname val@sp.bg_sd\endcsname{94}
\expandafter\def\csname val@sp.cal.big_hi\endcsname{2,619}
\expandafter\def\csname val@sp.cal.big_lo\endcsname{2,040}
\expandafter\def\csname val@sp.cal.method\endcsname{inprocess-2}
\expandafter\def\csname val@sp.cal.n_unstable\endcsname{1}
\expandafter\def\csname val@sp.cal.small_hi\endcsname{3,849}
\expandafter\def\csname val@sp.cal.small_lo\endcsname{3,642}
\expandafter\def\csname val@sp.cal_id\endcsname{pravaha-calibrate\_2026-11-08T09:53}
\expandafter\def\csname val@sp.cuda\endcsname{13.0}
\expandafter\def\csname val@sp.driver\endcsname{580.159.03}
\expandafter\def\csname val@sp.e4.bpt\endcsname{2,049}
\expandafter\def\csname val@sp.e4.dir_diff\endcsname{0.00}
\expandafter\def\csname val@sp.e4.r2\endcsname{0.9999}
\expandafter\def\csname val@sp.e6.device_pct\endcsname{0.6}
\expandafter\def\csname val@sp.e6.max_pct\endcsname{6.5}
\expandafter\def\csname val@sp.e7.malloc_extra_mb\endcsname{108}
\expandafter\def\csname val@sp.e7.malloc_w\endcsname{15.1}
\expandafter\def\csname val@sp.e7.read_max\endcsname{0.43}
\expandafter\def\csname val@sp.e7.write_max\endcsname{0.05}
\expandafter\def\csname val@sp.kernel\endcsname{6.17.0-1026-nvidia}
\expandafter\def\csname val@sp.n1.combined_err\endcsname{0.05}
\expandafter\def\csname val@sp.n1.copy_err\endcsname{0.06}
\expandafter\def\csname val@sp.n1.read_err\endcsname{0.14}
\expandafter\def\csname val@sp.n1.write_err\endcsname{0.08}
\expandafter\def\csname val@sp.n4.gb\endcsname{17.2}
\expandafter\def\csname val@sp.n4.max\endcsname{424}
\expandafter\def\csname val@sp.n4.min\endcsname{-977}
\expandafter\def\csname val@sp.n5.d2d\endcsname{-43}
\expandafter\def\csname val@sp.n5.d2h\endcsname{2,048}
\expandafter\def\csname val@sp.n5.h2d\endcsname{2,048}
\expandafter\def\csname val@sp.n6.bytes_per_txn\endcsname{2,028}
\expandafter\def\csname val@sp.n6.calibration\endcsname{2,071}
\expandafter\def\csname val@sp.n6.deviation_pct\endcsname{2.1}
\expandafter\def\csname val@sp.n6.run_spread_pct\endcsname{0.12}
\expandafter\def\csname val@sp.n6.status\endcsname{FAIL}
\expandafter\def\csname val@sp.n6.tolerance_pct\endcsname{0.44}
\expandafter\def\csname val@sp.n7.max_pct\endcsname{0.19}
\expandafter\def\csname val@sp.n8.diff_pct\endcsname{0.06}
\expandafter\def\csname val@sp.n_boots\endcsname{1}
\expandafter\def\csname val@sp.n_campaigns\endcsname{1}
\expandafter\def\csname val@sp.n_candidates\endcsname{7}
\expandafter\def\csname val@sp.product\endcsname{NVIDIA DGX Spark}
\expandafter\def\csname val@sp.unit\endcsname{smmuv3\_pmcg\_13002}
\makeatother


==> values_v4.tex <==
% AUTO-GENERATED by scripts/make_values_v4.py from data/v4/. Do not edit.
\makeatletter
\providecommand{\val}[1]{\@ifundefined{val@#1}{\textbf{??\detokenize{#1}??}}{\csname val@#1\endcsname}}
\expandafter\def\csname val@clk.int_obs\endcsname{22}
\expandafter\def\csname val@clk.int_req\endcsname{10}
\expandafter\def\csname val@clk.offset\endcsname{528}
\expandafter\def\csname val@clk.spread\endcsname{648}
\expandafter\def\csname val@d2d.c2c\endcsname{8.8}
\expandafter\def\csname val@llm.decode_gbs\endcsname{226}
\expandafter\def\csname val@llm.decode_gib_tok\endcsname{13.47}
\expandafter\def\csname val@llm.decode_s\endcsname{12.8}
\expandafter\def\csname val@llm.decode_tok_s\endcsname{15.5}
\expandafter\def\csname val@llm.gen_tokens\endcsname{200}
\expandafter\def\csname val@llm.idle_kread\endcsname{0.15}
\expandafter\def\csname val@llm.prefill_gbs\endcsname{125}
\expandafter\def\csname val@llm.prefill_kread\endcsname{38.2}
\expandafter\def\csname val@llm.prefill_kwrite\endcsname{7.9}
\expandafter\def\csname val@llm.prefill_passes\endcsname{2.9}
\expandafter\def\csname val@llm.prefill_s\endcsname{0.40}
\expandafter\def\csname val@llm.prompt_tokens\endcsname{1,510}
\expandafter\def\csname val@mis.embed\endcsname{0.25}
\expandafter\def\csname val@mis.kv_gib_tok\endcsname{0.20}
\expandafter\def\csname val@mis.kv_kib\endcsname{128}
\expandafter\def\csname val@mis.long_expect\endcsname{13.45}
\expandafter\def\csname val@mis.short_expect\endcsname{13.25}
\expandafter\def\csname val@mis.short_gib_tok\endcsname{13.26}
\expandafter\def\csname val@mis.weights\endcsname{13.50}
\expandafter\def\csname val@ovh.max\endcsname{0.53}
\expandafter\def\csname val@ovh.runs\endcsname{20}
\expandafter\def\csname val@ovh.spread\endcsname{2}
\expandafter\def\csname val@pt.known\endcsname{4}
\expandafter\def\csname val@pt.measured\endcsname{3.9999}
\expandafter\def\csname val@qwen.gib_tok\endcsname{7.52}
\expandafter\def\csname val@qwen.weights\endcsname{7.49}
\expandafter\def\csname val@reuse.mib\endcsname{16}
\expandafter\def\csname val@reuse.ratio\endcsname{0.0012}
\expandafter\def\csname val@smmu.bpt_hi\endcsname{3,690}
\expandafter\def\csname val@smmu.bpt_lo\endcsname{2,055}
\expandafter\def\csname val@smmu.n_gpu\endcsname{7}
\expandafter\def\csname val@smmu.n_total\endcsname{17}
\expandafter\def\csname val@smmu.saw_hi\endcsname{2,969}
\expandafter\def\csname val@smmu.thp\endcsname{10}
\expandafter\def\csname val@split.hi\endcsname{2.0158}
\expandafter\def\csname val@split.lo\endcsname{2.0141}
\expandafter\def\csname val@split.startup\endcsname{15}
\expandafter\def\csname val@ver.gn.d2h\endcsname{1.0000}
\expandafter\def\csname val@ver.gn.d2h.err\endcsname{0.00}
\expandafter\def\csname val@ver.gn.h2d\endcsname{1.0000}
\expandafter\def\csname val@ver.gn.h2d.err\endcsname{0.00}
\expandafter\def\csname val@ver.gn.maxerr\endcsname{0.28}
\expandafter\def\csname val@ver.gn.read\endcsname{0.9972}
\expandafter\def\csname val@ver.gn.read.err\endcsname{0.28}
\expandafter\def\csname val@ver.gn.write\endcsname{1.0000}
\expandafter\def\csname val@ver.gn.write.err\endcsname{0.00}
\expandafter\def\csname val@ver.size.d2h\endcsname{2}
\expandafter\def\csname val@ver.size.h2d\endcsname{2}
\expandafter\def\csname val@ver.size.read\endcsname{4}
\expandafter\def\csname val@ver.size.write\endcsname{4}
\expandafter\def\csname val@ver.sp.d2h\endcsname{1.0000}
\expandafter\def\csname val@ver.sp.d2h.err\endcsname{0.00}
\expandafter\def\csname val@ver.sp.h2d\endcsname{1.0000}
\expandafter\def\csname val@ver.sp.h2d.err\endcsname{0.00}
\expandafter\def\csname val@ver.sp.maxerr\endcsname{0.00}
\expandafter\def\csname val@ver.sp.read\endcsname{1.0000}
\expandafter\def\csname val@ver.sp.read.err\endcsname{0.00}
\expandafter\def\csname val@ver.sp.write\endcsname{1.0000}
\expandafter\def\csname val@ver.sp.write.err\endcsname{0.00}
\expandafter\def\csname val@ver.tol.d2h\endcsname{0.2}
\expandafter\def\csname val@ver.tol.h2d\endcsname{0.2}
\expandafter\def\csname val@ver.tol.read\endcsname{2.0}
\expandafter\def\csname val@ver.tol.write\endcsname{1.0}
\makeatother

